The McDonald Accelerating Stars Survey (MASS): White Dwarf Companions Accelerating the Sun-like Stars 12 Psc and HD 159062

We present the discovery of a white dwarf companion to the G1 V star 12 Psc found as part of a Keck adaptive optics imaging survey of long-term accelerating stars from the McDonald Observatory Planet Search Program. Twenty years of precise radial-velocity monitoring of 12 Psc with the Tull Spectrograph at the Harlan J. Smith telescope reveals a moderate radial acceleration ($\approx$10 m s$^{-1}$ yr $^{-1}$), which together with relative astrometry from Keck/NIRC2 and the astrometric acceleration between $Hipparcos$ and $Gaia$ DR2 yields a dynamical mass of $M_B$ = 0.605$^{+0.021}_{-0.022}$ $M_{\odot}$ for 12 Psc B, a semi-major axis of 40$^{+2}_{-4}$ AU, and an eccentricity of 0.84$\pm$0.08. We also report an updated orbit fit of the white dwarf companion to the metal-poor (but barium-rich) G9 V dwarf HD 159062 based on new radial velocity observations from the High-Resolution Spectrograph at the Hobby-Eberly Telescope and astrometry from Keck/NIRC2. A joint fit of the available relative astrometry, radial velocities, and tangential astrometric acceleration yields a dynamical mass of $M_B$ = 0.609$^{+0.010}_{-0.011}$ $M_{\odot}$ for HD 159062 B, a semi-major axis of 60$^{+5}_{-7}$ AU, and preference for circular orbits ($e$$<$0.42 at 95% confidence). 12 Psc B and HD 159062 B join a small list of resolved "Sirius-like" benchmark white dwarfs with precise dynamical mass measurements which serve as valuable tests of white dwarf mass-radius cooling models and probes of AGB wind accretion onto their main-sequence companions.

==> 12psc_rvs_tull.tex <==
\begin{deluxetable}{lcc}
\renewcommand\arraystretch{0.9}
\tabletypesize{\small}
\setlength{ \tabcolsep } {.1cm}
\tablewidth{0pt}
\tablecolumns{3}
\tablecaption{Tull Spectrograph Relative Radial Velocities of 12 Psc\label{tab:12psc_rvs}}
\tablehead{
    \colhead{Date}  & \colhead{RV} & \colhead{$\sigma_{\mathrm{RV}}$} \\
    \colhead{(BJD)} & \colhead{(m s$^{-1}$)} & \colhead{(m s$^{-1}$)}
        }
\startdata
%========================================================
%           Date    &          RV    &      RV_err   \\
%========================================================
   2452115.95277    &      -97.23    &        3.69   \\
   2452145.89854    &      -98.83    &        4.20   \\
   2452219.66771    &      -86.14    &        5.03   \\
   2452473.90774    &      -59.28    &        4.44   \\
   2452494.83891    &      -75.32    &        6.33   \\
   2452540.79863    &      -65.29    &        5.13   \\
   2452598.71506    &      -52.06    &        4.50   \\
   2452896.84418    &      -48.27    &        5.57   \\
   2452931.83102    &      -73.12    &        4.71   \\
   2453215.96238    &      -48.79    &        4.18   \\
   2453318.76599    &      -41.88    &        5.06   \\
   2453563.90794    &      -45.68    &        3.96   \\
   2453584.92356    &      -57.52    &        4.33   \\
   2453630.82851    &      -30.81    &        5.18   \\
   2453654.77953    &      -43.11    &        6.00   \\
   2453691.69398    &      -28.07    &        5.73   \\
   2453747.60632    &      -40.31    &        5.63   \\
   2453930.88437    &      -37.89    &        4.46   \\
   2453967.93127    &      -38.72    &        4.94   \\
   2453984.87585    &      -41.11    &        4.52   \\
   2454018.79889    &      -24.56    &        4.76   \\
   2454068.70451    &      -22.35    &        5.21   \\
   2454347.85739    &       -9.25    &        5.79   \\
   2454747.82589    &      -14.33    &        5.34   \\
   2455024.89834    &       -0.37    &        5.63   \\
   2455103.75934    &        2.95    &        8.45   \\
   2455153.71002    &        9.67    &        5.45   \\
   2455497.75119    &        1.33    &        6.09   \\
   2455587.55766    &        3.57    &        5.42   \\
   2455588.55221    &        7.29    &        5.24   \\
   2455758.87749    &       21.11    &        4.68   \\
   2455840.84134    &       11.43    &        5.55   \\
   2455910.65740    &       23.52    &        5.31   \\
   2456143.88515    &       17.37    &        5.39   \\
   2456177.89724    &       26.15    &        5.63   \\
   2456237.74312    &       17.67    &        6.13   \\
   2456522.89664    &       38.66    &        4.31   \\
   2456560.80009    &       39.60    &        4.81   \\
   2456590.78937    &       45.46    &        5.13   \\
   2456641.55108    &       56.07    &        4.71   \\
   2456884.85069    &       44.99    &        4.86   \\
   2456970.68181    &       50.29    &        5.04   \\
   2457005.56490    &       63.83    &        4.82   \\
   2457674.74673    &       74.08    &        5.25   \\
   2458040.76155    &       92.21    &        4.92   \\
   2458067.71366    &       94.59    &        4.45   \\
   2458322.92863    &       99.06    &        6.17   \\
   2458778.69077    &      111.90    &        4.65   \\
   2459055.92094    &      118.60    &        4.58   \\
   2459072.91387    &      108.89    &        5.41   \\
\enddata
\end{deluxetable}


==> hd159062_rvs_tull.tex <==
\begin{deluxetable}{lcc}
\renewcommand\arraystretch{0.9}
\tabletypesize{\small}
\setlength{ \tabcolsep } {.1cm}
\tablewidth{0pt}
\tablecolumns{3}
\tablecaption{HRS Relative Radial Velocities of HD 159062\label{tab:hd159062_rvs}}
\tablehead{
    \colhead{Date}  & \colhead{RV} & \colhead{$\sigma_{\mathrm{RV}}$} \\
    \colhead{(BJD)} & \colhead{(m s$^{-1}$)} & \colhead{(m s$^{-1}$)}
        }
\startdata
%========================================================
%           Date    &          RV    &      RV_err   \\
%========================================================
   2454698.72895    &       34.67    &        3.77   \\
   2454715.68103    &       45.29    &        3.29   \\
   2454726.62674    &       45.12    &        3.95   \\
   2454728.63730    &       35.47    &        3.13   \\
   2454873.01630    &       42.84    &        2.98   \\
   2454889.98057    &       39.49    &        3.39   \\
   2454918.88920    &       47.88    &        3.21   \\
   2455059.74200    &       19.49    &        3.33   \\
   2455100.63545    &       16.31    &        3.76   \\
   2455261.94792    &       15.50    &        2.62   \\
   2455281.89269    &       17.30    &        2.70   \\
   2455289.89143    &       13.48    &        3.01   \\
   2455289.89411    &       15.90    &        2.58   \\
   2455321.80285    &       14.29    &        3.87   \\
   2455321.80547    &       11.68    &        3.72   \\
   2455410.76655    &        8.58    &        3.67   \\
   2455410.76920    &        6.23    &        3.47   \\
   2455450.63568    &        8.28    &        3.54   \\
   2455450.63836    &       10.16    &        3.30   \\
   2455233.02598    &       17.94    &        2.38   \\
   2455598.02450    &        9.67    &        3.41   \\
   2455598.02718    &       10.34    &        3.56   \\
   2455599.02448    &        8.66    &        2.75   \\
   2455599.02716    &        9.12    &        2.90   \\
   2455603.02219    &        6.92    &        2.98   \\
   2455603.02486    &        3.26    &        3.03   \\
   2455632.91929    &        1.88    &        2.76   \\
   2455632.92196    &        2.96    &        3.07   \\
   2455690.77715    &        1.14    &        3.25   \\
   2455690.77983    &        1.79    &        3.78   \\
   2455724.68552    &       -6.20    &        3.41   \\
   2455724.68820    &       -2.46    &        3.52   \\
   2455754.82365    &       -4.92    &        4.10   \\
   2455754.82633    &       -4.08    &        3.88   \\
   2455989.96100    &       -2.17    &        3.20   \\
   2455989.96367    &       -9.17    &        2.95   \\
   2456010.89520    &       -2.97    &        2.93   \\
   2456010.89787    &       -6.79    &        2.69   \\
   2456030.87269    &       -1.83    &        7.47   \\
   2456030.87535    &        6.92    &        8.86   \\
   2456035.82667    &      -15.30    &        3.98   \\
   2456035.82935    &       -9.73    &        4.26   \\
   2456063.76733    &       -8.82    &        3.35   \\
   2456063.77000    &      -11.36    &        3.08   \\
   2456083.71678    &      -18.33    &        3.82   \\
   2456083.71945    &      -15.98    &        3.72   \\
   2456146.76630    &      -14.84    &        3.18   \\
   2456146.76897    &      -10.54    &        3.18   \\
   2456168.70828    &      -18.13    &        3.49   \\
   2456168.71095    &      -17.97    &        3.88   \\
   2456188.65554    &      -25.38    &        3.47   \\
   2456188.65822    &      -19.67    &        3.53   \\
   2456354.94963    &      -24.57    &        3.20   \\
   2456354.95230    &      -18.76    &        2.91   \\
   2456377.89506    &      -21.49    &        2.87   \\
   2456377.89946    &      -24.11    &        2.72   \\
   2456384.85232    &      -19.60    &        3.41   \\
   2456384.85498    &      -23.89    &        3.31   \\
   2456416.79746    &      -27.22    &        3.64   \\
   2456416.80013    &      -24.46    &        3.80   \\
   2456448.70171    &      -30.91    &        3.61   \\
   2456448.70438    &      -29.93    &        3.68   \\
   2456506.76401    &      -27.65    &        5.12   \\
   2456506.76668    &      -29.28    &        5.05   \\
\enddata
\end{deluxetable}

